Superconducting phases and the second Josephson harmonic in tunnel junctions between diffusive superconductors

We consider a planar SIS-type Josephson junction between diffusive superconductors (S) through an insulating tunnel interface (I). We construct fully self-consistent perturbation theory with respect to the interface conductance. As a result, we find correction to the first Josephson harmonic and calculate the second Josephson harmonic. At arbitrary temperatures, we correct previous results for the nonsinusoidal current-phase relation in Josephson tunnel junctions, which were obtained with the help of conjectured form of solution. Our perturbation theory also describes the difference between the phases of the order parameter and of the anomalous Green functions.

==> bib.bbl.tex <==

@article{Usadel1970,
title={Generalized Diffusion Equation for Superconducting Alloys},
author={Klaus D. Usadel},
journal={Phys. Rev. Lett.},
volume={25},
pages={507},
year={1970},
doi={10.1103/PhysRevLett.25.507}
}

@article{GK2005,
title={The Current Phase Relation in {Josephson} Tunnel Junctions},
author={A. A. Golubov and M. {\relax Yu}. Kupriyanov},
journal={JETP Lett.},
volume={81},
pages={335-341},
year={2005},
doi={10.1134/1.1944074},
 note = {[Pis’ma Zh. Eksp. Teor. Fiz., \textbf{81}, 419 (2005)]}
}

@article{Kupriyanov1992,
title={Effect of a finite transmission of the insulating layer on the properties of {SIS} tunnel junctions},
author={M. {\relax Yu}. Kupriyanov},
journal={JETP Lett.},
volume={56},
pages={399-404},
year={1992},
doi={},
note = {[Pis’ma Zh. Eksp. Teor. Fiz., \textbf{56}, 414 (1992)]}
}

@book{Abrikosov1988,
author={A. A. Abrikosov}, title={{Fundamentals of the Theory of Metals}}, publisher={NorthHolland, Amsterdam}, year={1988}
}


@book{Svidzinsky1982,
author={A. V. Svidzinsky}, title={{Spatially Non-Uniform Problems in the Theory of
Superconductivity}}, publisher={Nauka, Moscow}, year={1982},
note = {[in Russian]}
}

@article{KL1987,
title={Influence of boundary transparency on the critical current of ``dirty'' {SS'S} structures },
author={M. {\relax Yu}. Kuprianov and V. F. Lukichev },
journal={JETP},
volume={94},
pages={1163-1168},
year={1987},
doi={},
note = {[Zh. Eksp. Teor. Fiz., \textbf{94}, 139 (1987)]}
}

@article{PhysRevB.83.139901,
  title = {Spin-dependent boundary conditions for isotropic superconducting Green's functions},
  author = {Cottet, Audrey and Huertas-Hernando, Daniel and Belzig, Wolfgang and Nazarov, Yuli V.},
  journal = {Phys. Rev. B},
  volume = {83},
  issue = {13},
  pages = {139901(E)},
  numpages = {1},
  year = {2011},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.83.139901},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.83.139901}
}


@article{Belzig1999,
title={Quasiclassical {Green}’s function approach to mesoscopic superconductivity},
author={Wolfgang Belzig and Frank K. Wilhelm and Christoph Bruder and Gerd Sch{\"o}n and Andrei D. Zaikin},
journal={Superlattices Microstruct.},
volume={25},
pages={1251-1288},
year={1999},
doi={10.1006/spmi.1999.0710}}


% \cite{[][{ [JETP Lett. \textbf{74}, 96 (2001)].}]Fominov2001RusEng}

@BOOK{TinkhamBook,
 AUTHOR    = "M. Tinkham",
 TITLE     = "Introduction to Superconductivity (2nd edition)",
 PUBLISHER = "Dover",
 ADDRESS   = "New York",
 YEAR      = "2004",
%NOTE      = "",
 LANGUAGE  = "english"
}
@BOOK{AGDBookEng,
 AUTHOR    = "A. A. Abrikosov and L. P. Gor'kov and I. E. Dzyaloshinski",
 TITLE     = "Methods of Quantum Field Theory in Statistical Physics",
 PUBLISHER = "Dover",
 ADDRESS   = "New York",
 YEAR      = "1977",
%NOTE      = "",
 LANGUAGE  = "english"
}
@ARTICLE{Zaikin1981Eng,
 AUTHOR    = "A. D. Zaikin and G. F. Zharkov",
 TITLE     = "Theory of wide dirty \textit{SNS} junctions",
 JOURNAL   = "Sov. J. Low Temp. Phys.",
 VOLUME    = "7",
 PAGES     = "184--185",
 YEAR      = "1981",
 NOTE      = "[Fiz. Nizk. Temp., \textbf{7}, 375 (1981)]",
% LANGUAGE  = "english"
}
@article{Stoof1996.PhysRevB.53.14496,
  title = {Kinetic-equation approach to diffusive superconducting hybrid devices},
  author = {Stoof, T. H. and Nazarov, {\relax Yu}. V.},
  journal = {Phys. Rev. B},
  volume = {53},
  issue = {21},
  pages = {14496--14505},
  numpages = {0},
  year = {1996},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.53.14496},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.53.14496}
}
@ARTICLE{Golubov2002Eng,
 AUTHOR    = "A. A. Golubov and M. {\relax Yu}. Kupriyanov and {\relax Ya}. V. Fominov",
 TITLE     = "Critical current in {SFIFS} junctions",
 JOURNAL   = "JETP Lett.",
 VOLUME    = "75",
 PAGES     = "190",
 YEAR      = "2002",
 DOI = "10.1134/1.1475721",
note = {[Pis’ma Zh. Eksp. Teor. Fiz., \textbf{75}, 223 (2002)]}
}
@ARTICLE{Josephson1962,
 AUTHOR    = "B. D. Josephson",
 TITLE     = "Possible new effects in superconductive tunnelling",
 JOURNAL   = "Phys. Letters",
 VOLUME    = "1",
 PAGES     = "251",
 YEAR      = "1962",
  doi = "10.1016/0031-9163(62)91369-0",
%NOTE      = "",
 LANGUAGE  = "english"
}
@ARTICLE{Ambegaokar1963,
 AUTHOR    = "V. Ambegaokar and A. Baratoff",
 TITLE     = "Tunneling Between Superconductors",
 JOURNAL   = "Phys. Rev. Lett.",
 VOLUME    = "10",
 PAGES     = "486",
 YEAR      = "1963",
DOI = "10.1103/PhysRevLett.10.486",
%NOTE      = "",
 LANGUAGE  = "english"
}

@article{Likharev1979.RevModPhys.51.101,
  title = {Superconducting weak links},
  author = {Likharev, K. K.},
  journal = {Rev. Mod. Phys.},
  volume = {51},
  issue = {1},
  pages = {101--159},
  numpages = {0},
  year = {1979},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.51.101},
  url = {https://link.aps.org/doi/10.1103/RevModPhys.51.101}
}
@ARTICLE{Golubov2004review,
 AUTHOR    = "A. A. Golubov and M. {\relax Yu}. Kupriyanov and E. Il'ichev",
 TITLE     = "The current-phase relation in {Josephson} junctions",
 JOURNAL   = "Rev. Mod. Phys.",
 VOLUME    = "76",
 PAGES     = "411--469",
 YEAR      = "2004",
  month = "Apr",
  publisher = "American Physical Society",
  doi = "10.1103/RevModPhys.76.411",
  url = "https://link.aps.org/doi/10.1103/RevModPhys.76.411",
%NOTE      = "",
 LANGUAGE  = "english"
}
@ARTICLE{Ivanov1981Eng,
 AUTHOR    = "Z. G. Ivanov and M. {\relax Yu}. Kupriyanov and K. K. Likharev and S. V. Meriakri and O. V. Snigirev",
 TITLE     = "Boundary conditions for the {Usadel} and {Eilenberger} equations, and properties of ``dirty'' \textit{SNS} sandwich-type junctions",
 JOURNAL   = "Sov. J. Low Temp. Phys.",
 VOLUME    = "7",
 PAGES     = "274",
 YEAR      = "1981",
 NOTE      = "[Fiz. Nizk. Temp., \textbf{7}, 560 (1981)]"
 LANGUAGE  = "english"
}
@ARTICLE{Kupriyanov1982Eng,
 AUTHOR    = "M. {\relax Yu}. Kupriyanov and V. F. Lukichev",
 TITLE     = "The proximity effect in electrodes and the steady-state properties of {Josephson} \textit{SNS} structures",
 JOURNAL   = "Sov. J. Low Temp. Phys.",
 VOLUME    = "8",
 PAGES     = "526--529",
 YEAR      = "1982",
 NOTE      = "[Fiz. Nizk. Temp., \textbf{8}, 1045 (1982)]"
 LANGUAGE  = "english"
}
@ARTICLE{Zubkov1983Eng,
 AUTHOR    = "A. A. Zubkov and M. {\relax Yu}. Kupriyanov",
 TITLE     = "Influence of depairing in electrodes on the steady-state properties of weak links",
 JOURNAL   = "Sov. J. Low Temp. Phys.",
 VOLUME    = "9",
 PAGES     = "279--281",
 YEAR      = "1983",
 NOTE      = "[Fiz. Nizk. Temp., \textbf{9}, 548 (1983)]"
 LANGUAGE  = "english"
}
@article{Barash2012.PhysRevB.85.100503,
  title = {Anharmonic {Josephson} current in junctions with an interface pair breaking},
  author = {Barash, {\relax Yu}. S.},
  journal = {Phys. Rev. B},
  volume = {85},
  issue = {10},
  pages = {100503},
  numpages = {5},
  year = {2012},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.85.100503},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.85.100503}
}
@ARTICLE{Barash2014Eng,
 AUTHOR    = "{\relax Yu}. S. Barash",
 TITLE     = "Interfacial Pair Breaking and Planar Weak Links with an Anharmonic Current--Phase Relation",
 JOURNAL   = "JETP Lett.",
 VOLUME    = "100",
 PAGES     = "205--215",
 YEAR      = "2014",
 doi = {10.1134/S0021364014150041},
 note = {[Pis’ma Zh. Eksp. Teor. Fiz., \textbf{100}, 226 (2014)]}
}
@article{Sols1994.PhysRevB.49.15913,
  title = {Crossover from the {Josephson} effect to bulk superconducting flow},
  author = {Sols, Fernando and Ferrer, Jaime},
  journal = {Phys. Rev. B},
  volume = {49},
  issue = {22},
  pages = {15913--15919},
  year = {1994},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.49.15913},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.49.15913}
}
@article{Pastukh2017,
author = {Pastukh, O. {\relax Yu}.  and Shutovskii, A. M.  and Sakhnyuk, V. E. },
title = {The effect of depairing on the current-phase relation in {SIS} junctions in the presence of nonmagnetic impurities of arbitrary concentration},
journal = {Low Temp. Phys.},
volume = {43},
number = {6},
pages = {664--669},
year = {2017},
doi = {10.1063/1.4985972},
URL = {https://doi.org/10.1063/1.4985972},
note={[Fiz. Nizk. Temp. \textbf{43}, 835 (2017)]}
%eprint = {https://doi.org/10.1063/1.4985972}
}
@ARTICLE{Furusaki1991,
 AUTHOR    = "Akira Furusaki and Masaru Tsukada",
 TITLE     = "{DC} {Josephson} effect and {Andreev} reflection",
 JOURNAL   = "Solid State Commun.",
 VOLUME    = "78",
 NUMBER = "4",
 PAGES     = "299--302",
 YEAR      = "1991",
 DOI = "10.1016/0038-1098(91)90201-6",
%NOTE      = "",
 LANGUAGE  = "english"
}
@article{Bagwell1994.PhysRevB.49.6841,
  title = {Critical current of a one-dimensional superconductor},
  author = {Bagwell, Philip F.},
  journal = {Phys. Rev. B},
  volume = {49},
  issue = {10},
  pages = {6841--6846},
  numpages = {0},
  year = {1994},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.49.6841},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.49.6841}
}
@ARTICLE{Nazarov1999,
 AUTHOR    = "{\relax Yu}li V. Nazarov",
 TITLE     = "Novel circuit theory of {Andreev} reflection",
 JOURNAL   = "Superlattices Microstruct.",
 VOLUME    = "25",
 PAGES     = "1221",
 YEAR      = "1999",
 DOI = "10.1006/spmi.1999.0738"
%NOTE      = "",
 LANGUAGE  = "english"
